Nearly-Optimal Mergesorts: Fast, Practical Sorting Methods That Optimally Adapt to Existing Runs

We present two stable mergesort variants, "peeksort" and "powersort", that exploit existing runs and find nearly-optimal merging orders with practically negligible overhead. Previous methods either require substantial effort for determining the merging order (Takaoka 2009; Barbay & Navarro 2013) or do not have a constant-factor optimal worst-case guarantee (Peters 2001; Auger, Nicaud & Pivoteau 2015; Buss & Knop 2018). We demonstrate that our methods are competitive in terms of running time with state-of-the-art implementations of stable sorting methods.

==> preamble.tex <==
\makeatletter
\usepackage{lmodern}
\usepackage[T1]{fontenc}

\usepackage{babel}
\input{ushyphex.tex} % hyphenation exceptions


\newcommand{\ifarxiv}[2]{\ifthenelse{\equal{\version}{arxiv}}{#1}{#2}}
%
%


\usepackage{amsmath,amsfonts,amssymb,mathtools,nicefrac}
\usepackage{mleftright}\mleftright % redefine left and right to not add space around braces
\usepackage{relsize,ifthen,xspace,booktabs,adjustbox,needspace}
\usepackage{graphicx}


\usepackage{tikz}
\usetikzlibrary{patterns,calc,positioning}

%%%%% pseudocode algorithms
\usepackage{clrscode3e}
\def\Foreach{\kw{for each} }
\def\EndFor{\End\li\kw{end for} }
\def\EndIf{\End\li\kw{end if} }
\def\EndWhile{\End\li\kw{end while} }

%
%
%
%
%
\newenvironment{algorithm}[1][]{%
	\begin{table}[tbh]%
	\renewcommand*\tablename{Algorithm}
}{%
	\end{table}%
}


%
\hypersetup{
	final,
	unicode=true, 
	bookmarks=true,
	bookmarksnumbered=true,
	bookmarksdepth=2,
	bookmarksopen=true,
	breaklinks=true,
	hidelinks,
	pdfhighlight={/P}
}
%


%
%
%
%
%


\usepackage[american]{wref}


%
%




%
%
%
%
%
%
%
%
%%
%%
%
%%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
%
%
%
%
%
%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%   H E L P E R   C O M M A N D S   %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% temp-length, used in various places
\newlength{\tmp}

\def\clap#1{\makebox[0pt][c]{#1}}

\newcommand\plaincenter[1]{\mbox{}\hfill#1\hfill\mbox{}}

%%%%% create an hbox of the given width height and depth
%%%%% beware, ugly TeX hack, may result in strange
%%%%% behavior
\def\makeboxwhd#1#2#3#4{\setbox0=\hbox{#4}%
\ht0=#2%
\dp0=#3%
\wd0=#1%
\box0%
}
\newcommand*{\vcenteredhbox}[1]{\begingroup
\setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}

%%%%% create an hbox of the size of #2, but insert #3
%%%%% #1 can be l, c or r and gives the horizontal position
\newdimen\makeboxdimen
%\setlength\fboxsep{-\fboxrule}
\newcommand\makeboxlike[3][l]{%
\setbox0=\hbox{#2}%
\global\makeboxdimen=\wd0%
\setbox1=\hbox{\makebox[\makeboxdimen][#1]{%
\makebox[0pt][#1]{#3}%
}}%
\ht1=\ht0%
\dp1=\dp0%
\box1%	
}

\newcommand\like[3][c]{%
	\mathchoice{%dis
		\makeboxlike[#1]{%
			\ensuremath{\displaystyle\relax#2}%
		}{%
			\ensuremath{\displaystyle\relax#3}%
		}%
	}{%txt
		\makeboxlike[#1]{%
			\ensuremath{\textstyle\relax#2}%
		}{%
			\ensuremath{\textstyle\relax#3}%
		}%
	}{%sc
		\makeboxlike[#1]{%
			\ensuremath{\scriptstyle\relax#2}%
		}{%
			\ensuremath{\scriptstyle\relax#3}%
		}%
	}{%scsc
		\makeboxlike[#1]{%
			\ensuremath{\scriptscriptstyle\relax#2}%
		}{%
			\ensuremath{\scriptscriptstyle\relax#3}%
		}%
	}
}



%    __  __                          
%   |  \/  | __ _  ___ _ __ ___  ___ 
%   | |\/| |/ _` |/ __| '__/ _ \/ __|
%   | |  | | (_| | (__| | | (_) \__ \
%   |_|  |_|\__,_|\___|_|  \___/|___/
%                                    


% Common phrases
\newcommand*\ie{\mbox{i.\hspace{.2ex}e.}}
\newcommand*\eg{\mbox{e.\hspace{.2ex}g.}}
\newcommand*\iid{\mbox{i.\hspace{.2ex}i.\hspace{.2ex}d.}\xspace}
\newcommand*\wrt{\mbox{w.\hspace{.2ex}r.\hspace{.2ex}t.}\xspace}
\newcommand*\aka{\mbox{a.\hspace{.2ex}k.\hspace{.2ex}a.}\xspace}
\newcommand*\withoutlossofgenerality{\mbox{w.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\Withoutlossofgenerality{\mbox{W.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\almostsurely{\mbox{a.\hspace{.2ex}s.}\xspace}
\newcommand*\whp{\mbox{w.\hspace{.2ex}h.\hspace{.2ex}p.}\xspace}


\newcommand\R{\mathbb R}
\newcommand\N{\mathbb N}
\newcommand\Z{\mathbb Z}
\newcommand\Q{\mathbb Q}
\renewcommand\C{\mathbb{C}}
\newcommand\Oh{O}
\def\.{\mskip1mu} 


\DeclareMathOperator\ld{ld}



\newcommand{\surroundedmath}[3]{% #1=mathrel/mathbin/etc #2=spacing #3=symbol
	\mathchoice{%display
		#1{#2{#3}#2}%
	}{%text
		#1{#3}%
	}{%script
		#1{#3}%
	}{%scriptsript
		#1{#3}%
	}%
}
\newcommand\rel[1]{\surroundedmath{\mathrel}{\:}{#1}}
\newcommand\wrel[1]{\surroundedmath{\mathrel}{\;}{#1}}
\newcommand\wwrel[1]{\surroundedmath{\mathrel}{\;\;}{#1}}
\newcommand\bin[1]{\surroundedmath{\mathbin}{\:}{#1}}
\newcommand\wbin[1]{\surroundedmath{\mathbin}{\;}{#1}}
\newcommand\wwbin[1]{\surroundedmath{\mathbin}{\;\;}{#1}}

\newcommand{\eqwithref}[2][c]{%
	\relwithref[#1]{#2}{=}%
}
\newcommand{\relwithref}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize\wref{#2}}}}{#3}}%
}
\newcommand{\relwithtext}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize#2}}}{#3}}%
}



\newcommand\leafnode[1]{%
	\tikz[baseline=(p.base)] \node[rectangle,draw,inner sep=1pt,minimum size=2.3ex] (p) {\smaller$#1$};%
}
\newcommand\internalnode[1]{%
	\tikz[baseline=(p.base)] \node[circle,draw,inner sep=1pt,minimum size=2ex] (p) {\smaller$#1$};%
}
\newcommand\internalnodescript[1]{%
	\scriptsize
	\tikz \node[circle,draw,inner sep=.5pt,minimum size=2ex] (p) {$\scriptstyle#1$};%
}




\makeatother

